Do Data Center Network Metrics Predict Application-Facing Performance?

Applications that run in large-scale data center networks (DCNs) rely on the DCN's ability to deliver application requests in a performant manner. DCNs expose a complex design and operational space, and network designers and operators care how different options along this space affect application performance. One might run controlled experiments and measure the corresponding application-facing performance, but such experiments become progressively infeasible at a large scale, and simulations risk yielding inaccurate or incomplete results. Instead, we show that we can predict application-facing performance through more easily measured network metrics. For example, network telemetry metrics (e.g., link utilization) can predict application-facing metrics (e.g., transfer latency). Through large-scale measurements of production networks, we study the correlation between the two types of metrics, and construct predictive, interpretable models that serve as a suggestive guideline to network designers and operators. We show that no single network metric is universally the best predictor (even though some prior work has focused on a single predictor). We found that simple linear models often have the lowest error, while queueing-based models are better in a few cases.

==> acks.tex <==
\section*{Acknowledgments}

Jianan 

==> best-afm-qr95.tex <==
\begin{table}[htb]
\small
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{\AFM / QoS Class}                              & \textbf{Low} & \textbf{Medium} & \textbf{High} \\ \hline
\textbf{1kb Median Tx. Latency}   & MAU              & MAU                 & MAU               \\ \hline
% \textbf{8kb Median Transfer Latency}   & MAU              & MAU                 & MAU               \\ \hline
\textbf{64kb Median Tx. Latency}  & MAU              & P5\_P95\_Dist       & X                 \\ \hline
% \textbf{256kb Median Transfer Latency} & MAU              & P5\_P95\_Dist       & X                 \\ \hline
\textbf{1kb Tail Tx. Latency}     & MAU              & MAU                 & X                 \\ \hline
% \textbf{8kb Tail Transfer Latency}     & MAU              & MAU                 & MAU               \\ \hline
\textbf{64kb Tail Tx. Latency}    & MAU              & MAU                 & X                 \\ \hline
% \textbf{256kb Tail Transfer Latency}   & MAU              & X                   & X                 \\ \hline
\end{tabular}
\\ X indicates that no \NLMs were able to produce high-accuracy predictions for the corresponding \AFM.
\caption{\small \NLMs with the highest prediction accuracy.}

\label{tab:best_nlm_qr95}
\end{table}

==> best-afm.tex <==
\begin{table}[H]
\small
\center
\begin{subtable}[h]{0.5\textwidth}
\center

\begin{tabular}{|l||c|c|c|}
\hline
\textbf{AFM $\downarrow$ / QoS Class $\rightarrow$}                              & \textbf{Low} & \textbf{Medium} & \textbf{High} \\ \hline \hline
\textbf{1kb Median Tx. Latency}   & MAU              & AAU                 & AAU               \\ \hline
% \textbf{8kb Median Transfer Latency}   & AAU              & AAU                 & AAU               \\ \hline
\textbf{64kb Median Tx. Latency}  & MAU              & AAU                 & MAU               \\ \hline
% \textbf{256kb Median Transfer Latency} & AAU              & MAU                 & MAU               \\ \hline
\textbf{1kb Tail Tx. Latency}     & P5\_P95\_Dist              & MAU                 & AAU               \\ \hline
% \textbf{8kb Tail Transfer Latency}     & P5\_P95\_Dist    & AAU                 & MAU               \\ \hline
\textbf{64kb Tail Tx. Latency}    & MAU              & MAU                 & X                 \\ \hline
% \textbf{256kb Tail Transfer Latency}   & P5\_P95\_Dist    & MAU                 & MAU               \\ \hline
\end{tabular}
\caption{QR50 predictions.}
\label{tab:best_nlm_qr50}
\end{subtable}

\begin{subtable}[h]{0.5\textwidth}
\center

\begin{tabular}{|l||c|c|c|}
\hline
\textbf{AFM $\downarrow$ / QoS Class $\rightarrow$}                              & \textbf{Low} & \textbf{Medium} & \textbf{High} \\ \hline \hline
\textbf{1kb Median Tx. Latency}   & MAU              & MAU                 & MAU               \\ \hline
% \textbf{8kb Median Transfer Latency}   & MAU              & MAU                 & MAU               \\ \hline
\textbf{64kb Median Tx. Latency}  & MAU              & P5\_P95\_Dist       & X                 \\ \hline
% \textbf{256kb Median Transfer Latency} & MAU              & P5\_P95\_Dist       & X                 \\ \hline
\textbf{1kb Tail Tx. Latency}     & MAU              & MAU                 & X                 \\ \hline
% \textbf{8kb Tail Transfer Latency}     & MAU              & MAU                 & MAU               \\ \hline
\textbf{64kb Tail Tx. Latency}    & MAU              & MAU                 & X                 \\ \hline
% \textbf{256kb Tail Transfer Latency}   & MAU              & X                   & X                 \\ \hline
\end{tabular}\caption{QR95 predictions.}
\label{tab:best_nlm_qr95}
\end{subtable}
\\ X indicates that no \NLMs were able to produce high-accuracy predictions for the corresponding \AFM.
\caption{\small \NLMs with the highest prediction accuracy.}
\label{tab:best_nlm}
\end{table}

==> combined_methodology_algo.tex <==
\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}[htb]
\scriptsize
\caption{Combined Methodology}\label{alg:two}
\KwIn{(\NLM, \AFM)[] (\textit{array of tuples})}
\KwOut{has\_knee(\textit{bool})\newline
model\_attr(model, quantile):\{slope, intercept, confidence\} 
(\textit{key,value pairs}) } 

models $\leftarrow$ [queueing, linear] \\
quantiles $\leftarrow$ [50, 75, 95]

$has\_knee, knee\_value$ = \textbf{Kneedle}((\NLM, \AFM)[])

% \If{$has\_knee$}
% {
% (\NLM, \AFM)[] = (\NLM, \AFM)[$\NLM \leq knee\_value$]
% }

\ForEach{(m, q) in (models, quantiles)}{
    \uIf{$has\_knee$} {
        model\_attr($m,q$) = \textbf{QuantileRegression}($m,q$, (\NLM, \AFM)[$\NLM \leq knee\_value$])
    }
    \Else{
        model\_attr($m,q$) = \textbf{QuantileRegression}($m,q$, (\NLM, \AFM)[])
    }
}
\label{algo:combined_methodology}
\end{algorithm}

==> limitations.tex <==
\subsection{Limitations of Existing Technologies}

\jeff{I think we should exclude this material, it seems redundant.}

An ideal model would provide fine-grained, highly-accurate \AFM predictions given a set of \NLM measurements.

While predicting \AFMs brings tremendous benefits to various stakeholders, existing technologies fall short of doing so for various reasons:
\begin{itemize}[leftmargin=.1in, noitemsep,topsep=0pt]
    \item \textbf{Packet-level simulators} like NS-3 don't scale well to fairly-sized networks.
    \item \textbf{Simplistic network models} don't capture the complexity of network behavior.
    \item \textbf{Simplistic application models} are mismatched with realistic workloads, especially at scale.
    \item \textbf{Network-level simulations} provide no direct predictions for \AFMs.
    \item \textbf{Measuring performance of specific applications} is limited to small set of applications, often small deployments.
    \item \textbf{Instrumenting real applications} face privacy and scale issues, as well as the same challenges above.
\end{itemize}

To overcome these limitations, we exploit our ability to directly measure the application-facing performance for a large subset of representative applications running in our fleet. 
% Combining this unique application-facing performance trace with network-level traces, this paper reports our efforts to study how network metrics affect application-facing performance.
The combination of rich, large-scale measurements on both the network layer and transport layer creates a rare and unique opportunity for us to extract fabric-wide models and insights that would be useful in many perspectives.
% , as mentioned in Section~\ref{sec:intro}. 

